OmniMem: Scalable and Adaptive Memory Retrieval for Long Video Generation

Autoregressive (AR) video generation extends videos by producing latent chunks sequentially, but scaling to long videos requires repeated access to a growing historical KV cache. Existing methods reduce this cost by truncating the KV cache or compressing it into implicit memory, but both lose explicit access to query-relevant historical details. We propose OmniMem, an explicit full-range memory retrieval framework that performs sparse KV retrieval over the historical cache. To make this practical for chunk-based AR video generation, OmniMem addresses two issues: (i) local bias in sparse KV selection and (ii) Union Explosion in memory access. Adaptive Window Exclusion removes local-window blocks from the selection candidates when sufficient long-range history is available, preserving the sparse budget for informative long-range retrieval. Query-Shared KV Selection reduces cross-query diversity, while Per-Head Scattered KV Access avoids expanding head-specific selections into a large selected KV buffer. This allows each attention head to retrieve non-contiguous KV blocks according to its own selection pattern. Experiments on long-video generation show that OmniMem improves Dynamic Degree by 52.3% and preserves strong consistency over strong baselines, while maintaining comparable memory usage.

==> figs/app_inter1.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/interactive1.pdf}
\caption{
\textbf{.}
}
\label{fig:app_inter1}
\end{figure*}

==> figs/diff_head_pattern.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.94\linewidth]{assets/diff_head_pattern.pdf}
\caption{
\textbf{Head pattern.}
}
\label{fig:head_pattern}
\end{figure*}

==> figs/union_explosion.tex <==
\begin{figure}[t]
    \centering
    \subfloat[Cross-query divergence within one head.]{
        \fbox{\rule{0pt}{1.35in} \rule{0.45\linewidth}{0pt}}
        \label{fig:union-cross-query}
    }
    \hfill
    \subfloat[Cross-head divergence across attention heads.]{
        \includegraphics[width=0.48\linewidth]{assets/union.png}
        \label{fig:union-cross-head}
    }
    \caption{
    \textbf{Union explosion in selection attention.}
    Different query groups within the same head and different attention heads select different historical KV blocks.
    The selected-block union therefore grows across both the query and head dimensions, increasing the memory-access and materialization cost of naive selected-KV buffering.
    }
    \label{fig:union-explosion}
\end{figure}

==> minipages/fig_1.tex <==
\begin{figure}[ht]
\begin{minipage}[t]{0.475\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{assets/tiled_gemm.pdf}
\captionof{figure}{Illustration for tiled GEMM for a single token. The input $X$ and weights $W$ are both tiled into $k$ partitions along input feature.}
\label{fig:gemm tile}
\end{minipage}
\hfill
\begin{minipage}[t]{0.475\textwidth}
\centering
\includegraphics[width=0.85\linewidth]{assets/tile_gemm_bench.pdf}
\captionof{figure}{Latency benchmark for tiled GEMM in FFN. Note that the y axis is $log2$ scale.}
\label{fig:gemm tile bench}
\end{minipage}
\end{figure}


==> tabs/diff_group_head.tex <==
\begin{table}[t]
\centering
\caption{Necessity of Progressive Exclusion. We vary the number of recent chunks excluded 
from the selection pool.}
\label{tab:abl-prog}
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lcccc}
\toprule
\textbf{Excluded Chunks} & \textbf{IQ} & \textbf{SC} & \textbf{BC}  & \textbf{CLIP}  \\
\midrule
1 chunk               & -- & -- & -- & -- \\
2 chunks    & -- & -- & -- & -- \\
3 chunks              & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table}
